Zonotope Domains for Lagrangian Neural Network Verification

Neural network verification aims to provide provable bounds for the output of a neural network for a given input range. Notable prior works in this domain have either generated bounds using abstract domains, which preserve some dependency between intermediate neurons in the network; or framed verification as an optimization problem and solved a relaxation using Lagrangian methods. A key drawback of the latter technique is that each neuron is treated independently, thereby ignoring important neuron interactions. We provide an approach that merges these two threads and uses zonotopes within a Lagrangian decomposition. Crucially, we can decompose the problem of verifying a deep neural network into the verification of many 2-layer neural networks. While each of these problems is provably hard, we provide efficient relaxation methods that are amenable to efficient dual ascent procedures. Our technique yields bounds that improve upon both linear programming and Lagrangian-based verification techniques in both time and bound tightness.

==> tex_files/experiments.tex <==
\section{Experiments}


We evaluate the effectiveness of our approach on several networks trained on the MNIST and CIFAR-10 datasets. While many state-of-the-art verification techniques employ a branch-and-bound strategy, we have thusfar only provided an innovation on the bounding component of this pipeline. As the choice of branching subroutine can be interchanged with various bounding algorithms and vice versa, we focus our evaluations only upon the improvement provided by our novel bounding algorithm, noting that it can be employed in a variety of branching schemes. To that end, the primary metric of interest will be the \emph{bound} provided by a single run of each competing algorithm, though for completeness, we do also evaluate verified robustness percentages on several MNIST networks. 

\paragraph{Dual Technique Bound Evaluation} 
We separate our experiments into the case where only the output neuron is optimized, and the case where every neuron is optimized to provide tighter intermediate box bounds. We compare both the bound and running time against the following approaches: \textbf{BDD+}, the Lagrangian Decomposition procedure proposed in \cite{Bunel2020-cl}, where the optimization is performed using optimal proximal step sizes; \textbf{LP}, the original linear programming relaxation using the PLANET relaxation on each ReLU neuron \cite{Zico_Kolter2017-va}; \textbf{Anderson}, the linear programming relaxation, where 1-cut is applied per neuron as in \cite{anderson2020strong}; \textbf{AS}, a recent Lagrangian technique which iteratively chooses cuts to employ from the Anderson relaxation \cite{De_Palma2021-sp}. 
All competing techniques are run implemented using the code and hyperparameter choices from prior works. 
GPU acceleration is employed where applicable. 
A complete description of hyperparameter choices for these competing methods is contained in Appendix \ref{app:hyperparameters}.
Of these techniques, observe that only ours, Anderson, and the AS technique are capable of surpassing the stagewise LP technique, i.e. scaling the convex barrier. 

\paragraph{Single-stage Bound Evaluation:} 
In this setting, we consider three networks trained on the MNIST dataset and one trained on the CIFAR dataset. In the main paper, we highlight only the MNIST-Deep network and the CIFAR network; data from the other networks is contained in the supplementary. Networks and weights are taken from prior works. 


As we only consider scalar verification problems, for every example with label $i$, we compare the difference of the \(i\)\textsuperscript{th} and \((i+1)\)\textsuperscript{th} logit, e.g. comparing the 7\textsuperscript{th} vs 8\textsuperscript{th} logits on an MNIST network.
It is trivial to extend this procedure to a multi-class task by applying the verification \(n-1\) times for each incorrect logit.



In the single-stage setting, we make the following choices for the hyperparameters of our approach. 
We initialize the intermediate bounds using zonotopes informed by the boxes attained by the best of the \texttt{DeepZ} bounds and IBP bounds.
Then we decompose each zonotope into 2-dimensional partitions, which are dictated by the `similarity' heuristic for the fully-connected network, and the `spatial' heuristic for convolutional networks. 

Next we apply 1000 iterations of the Adam optimizer during the dual ascent procedure. 
We report the value at the last iteration as \textbf{ZD-2D} in the plots. Finally, we merge the partitions of only the last layer of each neuron, generating 20-dimensional zonotopes. The dual function is evaluated under this new partitioning and the values are reported in the figures as \textbf{ZD-MIP}. We merge this layer only because it is both the narrowest and has the largest contribution to the dual, and thus stands the most to gain by a coarser partitioning.

First we present the results of our method on the MNIST-Deep network, which has 5196 ReLU neurons, over a verification domain of $\ell_\infty$ boxes of radius \(0.1\), clipped to remain inside the valid range of images. 
\Cref{fig:mnist-deep-cdf} presents the distribution of reported bounds over every example in the MNIST validation set that the model classifies correctly.

We can see that even without using MIPs at the end, our technique can provide significantly tighter bounds than competing methods. 
Applying a fast MIP solver at the end of our dual ascent further improves the bound by a substantial margin.
Running times corresponding to this figure are presented in \cref{table:single-stage-mini}. 
We find that running times do not vary significantly between examples for the competing methods, and our approach takes only slightly longer than other dual approaches and is still highly scalable. We do, however, observe a larger variance in runtime during the final MIP evaluation phase. Some MIP subproblems might be significantly harder to solve than others, but since this only occurs during the evaluation phase, we could mitigate this by early-stopping the MIP and reporting the best bound.
\begin{figure}[!htb]
\begin{subfigure}{0.5\textwidth}
  \centering
    \resizebox{0.9\textwidth}{!}{\input{figures/mnist_deep_cdf.pgf}}
  \label{fig:mnist-deep-cdf}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
  \centering
    \resizebox{0.9\textwidth}{!}{\input{figures/cifar_sgd_cdf.pgf}}
  \label{fig:cifar_sgd_Cdf}
\end{subfigure}
    \caption{Cumulative density function plots of the bounds obtained by each algorithm for a deep convolutional network trained on MNIST (left) and a deep convolutional network trained on CIFAR10 (right). Lines further to the right indicate tighter lower bounds. Our algorithms are bolded in the legend.}
\end{figure}



\begin{wraptable}{r}{7cm}
\centering
\caption{Timing data for the single-stage setting.}\label{table:single-stage-mini}
\begin{tabular}{lrr}
\toprule
Alg\textbackslash{}Net & MNIST Deep & CIFAR SGD \\
\midrule
BDD+ & \(2.5 \pm 0.2\) & \(1.5 \pm 0.1\) \\
LP & \(4.8 \pm 0.5\) & \(6.2 \pm 0.6\) \\
\textbf{ZD-2D} & \(10.9 \pm 0.5\) & \(7.6 \pm 0.3\) \\
AS & \(16.9 \pm 1.2\) & \(10.2 \pm 0.8\) \\
\textbf{ZD-MIP} & \(23.1 \pm 12.4\) & \(11.0 \pm 3.1\) \\
Anderson & \(52.4 \pm 27.5\) & \(21.3 \pm 4.6\) \\
\bottomrule
\end{tabular}
\end{wraptable}
We present similar results in the single-stage setting for a CIFAR-10 network with 6244 ReLU neurons trained using SGD in \cref{fig:cifar-sgd-cdf}.
Here the input region is constrained to be an $\ell_\infty$-box of radius $\epsilon = 5/255$, mirroring the experimental setup of \cite{De_Palma2021-sp}. 
Again we see similar results that our approach is able to provide bounds that are noticeably tighter than previous techniques at a comparable runtime. 
% Similar plots and bounds are shown for a CIFAR network trained adversarially in the Appendix.

\paragraph{Stagewise Bound Evaluation: } 
Now we turn our attention to the setting where enough computation time is allowed to perform the optimization procedure on every neuron in turn, which is able to generate tighter box bounds.  Here we notice an interesting observation: our method can be improved by leveraging tighter intermediate box bounds, but is agnostic as to where these bounds come from. Indeed, our approach can take as input any collection of tighter box bounds and generate tighter zonotopes via Proposition \ref{prop:box-deepz}. 
However, our current implementation of this tighter primal bound is not vectorized to be amenable, in the way that others are, to stagewise bounding procedures. This is purely an implementation detail, and we instead use existing primal bounding techniques. 


In this setting, we compare against the linear programming approach, BDD+, and the Active Set approach with 256 and 512 iterations, denoted AS256, AS512. We leverage box bounds provided by each of the dual approaches to inform zonotope bounds and run our method, which we denote with a $\mathbf{\to\text{ZD}}$ in the figures. Note that BDD+ can never surpass the bounds provided by the linear programming approach, whereas ours and the active set procedure can both be improved with an improved computation time. Thus, it is not sufficient to only provide a better bound, but to do so in a shorter runtime. In this case, our approach performs 2000 iterations of Adam on 2-d zonotopes, and increases the partition size of the final two layers of each network to sizes of 16 and 20 respectively.

In \cref{fig:mnist-ffnet-all-cdf, fig:mnist-deep-all-cdf}, we present the bounds provided by the MNIST-FFNet and MNIST-Deep network, which have 960 and 5196 neurons respectively. Timing data is presented in \cref{table:all-stage-mini}. In both cases we notice that the BDD+ method completes very quickly and attains a bound only slightly worse than the LP bound. Our approach, when initialized with the BDD+ bounds runs more efficiently than the AS256 method, providing bounds that are comparable or better to the even more expensive AS512 approach. Indeed, we show that AS256 combined with our approach can improve upon \emph{both} the bounds and the runtime in almost every instance than the AS512 approach. The tightest bounds are attained when applying our result to the AS512 box bounds. These results show that it is often profitable to spend less time running the Active Set approach, instead decreasing the iterations and performing the relatively cheaper zonotope-based approach, where zonotope-based optimization is only applied to the final neuron. 


\begin{figure}[!htb]

\begin{subfigure}{0.5\textwidth}
  \centering
    \resizebox{0.9\textwidth}{!}{\input{figures/mnist_ffnet_all_cdf.pgf}}
  \label{fig:mnist_ffnent-all-cdf}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
  \centering
    \resizebox{0.9\textwidth}{!}{\input{figures/mnist_deep_all_cdf.pgf}}
  \label{fig:mnist-deep-all-cdf}
\end{subfigure}
\end{figure}



%\begin{wraptable}{r}{7cm}
%\centering
%\caption{Timing data for all-stage nets. see \cref{table:single-stage-mini} for format.}
%\centering
%\begin{tabular}{lrr}
%\toprule
%Alg\textbackslash{}Net & MNIST Deep & MNIST Wide \\
%\midrule
%BDD+ & \(15.4 \pm 0.4\) & \(8.3 \pm 0.3\) \\
%\textbf{BDD+ → ZD} & \(51.7 \pm 14.0\) & \(36.4 \pm 6.8\) \\
%AS256 & \(138.9 \pm 0.9\) & \(45.4 \pm 0.6\) \\
%\textbf{AS256 → ZD} & \(174.1 \pm 13.6\) & \(73.3 \pm 6.6\) \\
%AS512 & \(289.3 \pm 1.7\) & \(91.3 \pm 0.9\) \\
%\textbf{AS512 → ZD} & \(324.1 \pm 13.5\) & \(119.2 \pm 6.9\) \\
%LP & \(2132.2 \pm 494.4\) & \(387.1 \pm 65.5\) \\
%\bottomrule
%\end{tabular}
%\label{table:all-stage-mini}
%\end{wraptable}
%


% \begin{table}[!htb]
% \caption{Timing results for all-stage nets, see \cref{table:single-stage-mini} for format.}
% \centering
% \begin{tabular}{lrr}
% \toprule
% Alg\textbackslash{}Net & MNIST Deep & MNIST Wide \\
% \midrule
% BDD+ & \(15.4 \pm 0.4\) & \(8.3 \pm 0.3\) \\
% \textbf{BDD+ → ZD} & \(51.7 \pm 14.0\) & \(36.4 \pm 6.8\) \\
% AS256 & \(138.9 \pm 0.9\) & \(45.4 \pm 0.6\) \\
% \textbf{AS256 → ZD} & \(174.1 \pm 13.6\) & \(73.3 \pm 6.6\) \\
% AS512 & \(289.3 \pm 1.7\) & \(91.3 \pm 0.9\) \\
% \textbf{AS512 → ZD} & \(324.1 \pm 13.5\) & \(119.2 \pm 6.9\) \\
% LP & \(2132.2 \pm 494.4\) & \(387.1 \pm 65.5\) \\
% \bottomrule
% \end{tabular}
% \label{table:all-stage-mini}
% \end{table}
% 


\paragraph{\%-Verified Robustness:}
To evaluate in a more realistic setting we also consider our approach without any branching to evaluate percent-verified-robustness on MNIST networks. We mimic the experimental setup from \cite{wang2021beta, singh2019beyond, tjandraatmadja2020convex, muller2021precise} . These results are presented in Table \ref{table:pct-robust}. While our approach is not performing at state-of-the-art robustness levels, we observe that we are either faster or tighter than competing techniques that do not leverage branching. Since a branched variant of BDD+ is tighter than all but $\beta$-CROWN, we conjecture the same behaviour for ZD if we were to apply it into a branch-and-bound pipeline. 
\begin{table}[]
\caption{Verified Robustness on MNIST Networks. Methods denoted with an asterisk had numbers taken from \cite{wang2021beta}. Note that $\beta$-CROWN approach uses FSB branching, while other approaches do not. } 
\label{table:pct-robust}
\begin{tabular}{l|c|l|l|l|l|l}
Model     & $\epsilon$ & \textbf{ZD}         & BDD+         & CROWN*      & PRIMA*        & $\beta$-CROWN* \\ \hline
MLP 5x100 & 0.026    & 28.5\% (24s) & 19.8\% (7s)  & 16.0\% (1s) & 51.0\% (159s) & 69.9\% (102s)      \\
MLP 8x100 & 0.026    & 21.8\% (19s) & 19.1\% (15s) & 18.2\% (1s) & 42.8\% (301s) & 62.0\% (103s)      \\
MLP 5x200 & 0.015    & 41.8\% (28s) & 33.2\% (8s)  & 29.2\% (2s) & 69.0\% (224s) & 77.4\% (86s)       \\
MLP 8x200 & 0.015    & 29.7\% (26s) & 27.4\% (17s) & 25.9\% (6s) & 62.4\% (395s) & 73.5\% (95s)       \\
ConvSmall & 0.12     & 52.6\% (38s) & 16.6\% (6s)  & 15.8\% (3s) & 59.8\% (42s)  & 72.7\% (7s)       
\end{tabular}
\end{table}
